Multi-User Augmented Reality with Infrastructure-free Collaborative Localization

Multi-user augmented reality (AR) could someday empower first responders with the ability to see team members around corners and through walls. For this vision of people tracking in dynamic environments to be practical, we need a relative localization system that is nearly instantly available across wide-areas without any existing infrastructure or manual setup. In this paper, we present LocAR, an infrastructure-free 6-degrees-of-freedom (6DoF) localization system for AR applications that uses motion estimates and range measurements between users to establish an accurate relative coordinate system. We show that not only is it possible to perform collaborative localization without infrastructure or global coordinates, but that our approach provides nearly the same level of accuracy as fixed infrastructure approaches for AR teaming applications. LocAR uses visual-inertial odometry (VIO) in conjunction with ultra-wideband (UWB) ranging radios to estimate the relative position of each device in an ad-hoc manner. The system leverages a collaborative 6DoF particle filtering formulation that operates on sporadic messages exchanged between nearby users. Unlike map or landmark sharing approaches, this allows for collaborative AR sessions even if users do not overlap the same spaces. LocAR consists of an open-source UWB firmware and reference mobile phone application that can display the location of team members in real-time using mobile AR. We evaluate LocAR across multiple buildings under a wide-variety of conditions including a contiguous 30,000 square foot region spanning multiple floors and find that it achieves median geometric error in 3D of less than 1 meter between five users freely walking across 3 floors.

==> 1-2-Motivation.tex <==
\section{Background}
\subsection{Multi-user AR}

\subsection{Visual Inertial Odometry}

\subsection{Ultra Wideband Ranging}



==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $< | sed 's/^%\\citestyle{acmauthoryear}/\\citestyle{acmauthoryear}/'      > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst

